State of the Art of User Simulation approaches for conversational information retrieval

Conversational Information Retrieval (CIR) is an emerging field of Information Retrieval (IR) at the intersection of interactive IR and dialogue systems for open domain information needs. In order to optimize these interactions and enhance the user experience, it is necessary to improve IR models by taking into account sequential heterogeneous user-system interactions. Reinforcement learning has emerged as a paradigm particularly suited to optimize sequential decision making in many domains and has recently appeared in IR. However, training these systems by reinforcement learning on users is not feasible. One solution is to train IR systems on user simulations that model the behavior of real users. Our contribution is twofold: 1)reviewing the literature on user modeling and user simulation for information access, and 2) discussing the different research perspectives for user simulations in the context of CIR

==> 1modelisation.tex <==
The first user modeling approaches in IR were based on cognitive approaches \cite{Belkin1984CognitiveTransfer}. 

It produces a description of the users characterized by an objective or a problem as well as a knowledge of the world. It also describes the conditions necessary for an IR system to be effective with ambiguous queries. Many derivatives were then proposed  (e.g., ISP \cite{Kuhlthau:1991},  IS\&R \cite{Ingwersen:2005b},  Ellis \cite{Ellis:1989}).



Other works have focused on the statistical analysis of user logs to highlight typical user preferences or behaviors. \cite{Kelly2001ReadingInteraction} have linked user interactions to document relevance indicators. More recently, \cite{Chuklin2013ModelingPage} modeled user behavior towards results pages (e.g., users who go to the second result page tend to continue on subsequent result pages). 


However, modeling the behavior of user clicks is complex, because clicks are not a perfect indicator of the relevance of retrieved documents. Indeed, users can be victims of position bias \cite{Wang2018PositionSearch} or presentation bias \cite{Yue2010BeyondData} (some titles are more attractive due to the presence of images or keywords present in the query ). The diversity in user behavior also complicates modeling, for a same request, users do not have the same expectations and therefore do not have the same click behavior \cite{Hu2011CharacterizingModels}. Some statistical models are introduced to interpret user behavior. One of the first click models to estimate the probability of clicking on a document is the \textit{cascade} model \cite{Craswell2008AnModels}. Authors are limited to one click and assume that users scroll top to bottom through the retrieved list of documents until they find a relevant document. \cite{Chapelle2009ARanking} proposed a Bayesian model to estimate the relevance of documents according to user clicks, despite position bias. \cite{Agichtein2006ImprovingTerms} shows correlations between characteristics of user behavior and user satisfaction. \cite{Dupret2008AObservations} introduce the \textit{user browsing model} (UBM) which allows to estimate the click probability on a document of rank \textit{r} according to the rank \textit{r '} of the previously clicked document despite the positional bias.
\cite{Shen2012PersonalizedFiltering} model user behavior based on requests and documents while taking into account the bias induced by the variability of user behavior. 

 %La modélisation des comportements utilisateurs n'est pas limitée aux clics. 
%Certains travaux vont plus loin et tentent de modéliser les mouvements de la souris et le mouvement des yeux sur l'écran comme \cite{Liu2014FromSearch}. Elle utilise ce modèle pour faire du re-ranking.
Recently, many works are interested in understanding the intents of users with the objective of building conversational systems. These approaches have mainly focused on query reformulation.\cite{Zamani2020GeneratingRetrieval,Sordoni2015ASuggestion,DBLP:conf/circle/MustarLP20}.


==> content/1modelisation.tex <==
The first user modeling approaches in IR were based on cognitive approaches \cite{Belkin1984CognitiveTransfer}. 

It produces a description of the users characterized by an objective or a problem as well as a knowledge of the world. It also describes the conditions necessary for an IR system to be effective with ambiguous queries. Many derivatives were then proposed  (e.g., ISP \cite{Kuhlthau:1991},  IS\&R \cite{Ingwersen:2005b},  Ellis \cite{Ellis:1989}).



Other works have focused on the statistical analysis of user logs to highlight typical user preferences or behaviors. \cite{Kelly2001ReadingInteraction} have linked user interactions to document relevance indicators. More recently, \cite{Chuklin2013ModelingPage} modeled user behavior towards results pages (e.g., users who go to the second result page tend to continue on subsequent result pages). 


However, modeling the behavior of user clicks is complex, because clicks are not a perfect indicator of the relevance of retrieved documents. Indeed, users can be victims of position bias \cite{Wang2018PositionSearch} or presentation bias \cite{Yue2010BeyondData} (some titles are more attractive due to the presence of images or keywords present in the query ). The diversity in user behavior also complicates modeling, for a same request, users do not have the same expectations and therefore do not have the same click behavior \cite{Hu2011CharacterizingModels}. Some statistical models are introduced to interpret user behavior. One of the first click models to estimate the probability of clicking on a document is the \textit{cascade} model \cite{Craswell2008AnModels}. Authors are limited to one click and assume that users scroll top to bottom through the retrieved list of documents until they find a relevant document. \cite{Chapelle2009ARanking} proposed a Bayesian model to estimate the relevance of documents according to user clicks, despite position bias. \cite{Agichtein2006ImprovingTerms} shows correlations between characteristics of user behavior and user satisfaction. \cite{Dupret2008AObservations} introduce the \textit{user browsing model} (UBM) which allows to estimate the click probability on a document of rank \textit{r} according to the rank \textit{r '} of the previously clicked document despite the positional bias.
\cite{Shen2012PersonalizedFiltering} model user behavior based on requests and documents while taking into account the bias induced by the variability of user behavior. 

Recently, many works are interested in understanding users' intents with the objective of building conversational systems. These approaches have mainly focused on query reformulation.\cite{Zamani2020GeneratingRetrieval,Sordoni2015ASuggestion,DBLP:conf/circle/MustarLP20}.
 %La modélisation des comportements utilisateurs n'est pas limitée aux clics. 
%Certains travaux vont plus loin et tentent de modéliser les mouvements de la souris et le mouvement des yeux sur l'écran comme \cite{Liu2014FromSearch}. Elle utilise ce modèle pour faire du re-ranking.

